Cross-View-Prediction: Exploring Contrastive Feature for Hyperspectral Image Classification

This paper presents a self-supervised feature learning method for hyperspectral image classification. Our method tries to construct two different views of the raw hyperspectral image through a cross-representation learning method. And then to learn semantically consistent representation over the created views by contrastive learning method. Specifically, four cross-channel-prediction based augmentation methods are naturally designed to utilize the high dimension characteristic of hyperspectral data for the view construction. And the better representative features are learned by maximizing mutual information and minimizing conditional entropy across different views from our contrastive network. This 'Cross-View-Predicton' style is straightforward and gets the state-of-the-art performance of unsupervised classification with a simple SVM classifier.

==> past_version.tex <==
\begin{comment}
\section{Introduction}
With the rapid development of deep learning, much progress has been made in the hyperspectral classification field. Feature extraction is an essential part in the hyperspectral classification. And recent years, many great supervised deep learning methods for hyperspectral classification were good at feature extraction, such as one-dimensional convolutional neural networks (1DCNN) \cite{1D-CNN}, three-dimensional convolutional neural networks (3DCNN) \cite{3DCNN}, deep recurrent neural networks (RNN) \cite{RNN}, deep feature fusion network (DFFN) \cite{DFFN}, spectral-spatial residual network (SSRN) \cite{SSRN}, \dd{adaptive spectral-spatial multiscale contextual feature extraction \cite{adaptive}, fully contextual network (FullyContNet) \cite{contextual}, 3D attention denoising network \cite{Attention}}. \dr{Besides, some machine learning methods are also good at feature extraction, such as multitask learning-based reliability analysis \cite{multitask}, joint sparse representation and multitask learning \cite{jointsparse}. } Nowadays, it is widely admitted that the fusion of spatial information and spectral information is the best strategy to extract features for hyperspectral classification. Furthermore, deep learning models show great power in finding the two kinds of information. With enough labeled samples, many supervised learning methods can effectively learn the spatial and spectral information simultaneously (e.g., SSRN) and update the models' parameters, thus getting good hyperspectral classification results. 

However, there are some disadvantages to supervised learning methods. First, severe data dependence is the notorious disadvantage of supervised deep learning. Without enough labeled samples, many supervised deep learning methods work badly. Second, many supervised deep learning methods only rely on the labels to supervise the extraction of features. As a result, with the increase of labels, the models need to be retrained entirely, which seems expensive in the practical circumstances.

Researchers have paid their attention to unsupervised learning methods to avoid the disadvantages of supervised deep learning in the past years. Unsupervised learning methods are mostly feature extraction algorithms, with a suitable feature extractor, we can use a simple classifier to get good classification results. To some extent, unsupervised learning methods are more applicable in practical scenarios. For unsupervised learning, there are some classic methods widely applied to all kinds of fields, such as principal component analysis (PCA) \cite{PCA} and independent component analysis (ICA) \cite{ICA}. These traditional algorithms remain efficient in the pre-process or feature extraction field. 

Generally speaking, unsupervised learning aims to dig out information from data other than labels; there are two major ways to achieve the objective: representative learning and discriminative learning. There are two famous representative learning models: autoencoder (AE) \cite{AE} and generative adversarial network (GAN)  \cite{GAN}. The two methods both use the self-similarity of data and then construct a model that can map the original data to some certain distributions. In this way, we can get generated distributions which are similar to the distributions of real samples. As a result, we can get forgery samples that are similar to real samples or get good feature extractors. Inspired by autoencoder, stacked sparse autoencoder  (SSAE) \cite{SSAE} used autoencoder for sparse spectral feature learning and multiscale spatial feature learning, respectively and then fused these two kinds of feature for hyperspectral classification. Furthermore, GAN \cite{GANforC} has also been proved to be useful in extracting spectral-spatial features for hyperspectral classification. Except for these methods, three-dimensional convolutional autoencoder  (3DCAE) \cite{3DCAE}, semi-supervised GAN \cite{semi-GAN}, GAN-Assisted CapsNet  (TripleGAN) \cite{triple-gan} and many other papers also originated from the representative learning. Generally, many researchers have acknowledged the utility of the representative learning methods in the remote sensing field.

On the other hand, discriminative learning is also an original idea in exploring the information of data. \dd{Support vector machine (SVM) \cite{svm} may be the most classic discriminative learning algorithm, and decision tree \cite{dtree}, multilayer perceptron (MLP) \cite{mlp}, conditional random field (CRF) \cite{crf} are all methods based on discriminative learning. Among various discriminative learning models, an impressive method is the contrastive learning method.} Unlike autoencoder and GAN, the contrastive learning method does not care about the details of the data. It cares about the difference between the different samples. In other words, contrastive learning aims to discriminate different samples and does not aim to find samples' exact distributions. By comparing different samples, a discriminator is trained and can be used for classification or other tasks. By finding the difference between two randomly selected samples, the discriminator learns to extract features that are helpful for downstream tasks.\dd{ Contrastive learning can be applied in supervised \cite{sucontra} as well as unsupervised learning \cite{uncontra}.}\cite{steinwart2008support}

For unsupervised contrastive learning, there are no label information can be utilized at all. Therefore a paradigm is widely used for unsupervised learning: we use two kinds of data augmentation methods to transform a single sample into two transformed samples because contrastive learning requires the contrast between two samples. In this way, we introduce a kind of information: the two samples originate from the same sample. Then with a proper model structure and a well-designed objective function, we can train an encoder that can map the samples to latent encoding space, and the features from the encoding space can well represent the original samples. When the encoder acts as a feature extractor, many downstream tasks can be done. Much work has been done in the computer vision field, such as momentum contrast \cite{Moco} and a simple framework for contrastive learning \cite{simclr}. They proposed some original structures for unsupervised contrastive learning and got promising results in many visual datasets. Furthermore, prototypical contrastive learning (PCL) \cite{PCL} combined cluster algorithm with contrastive learning, and got better performances than other methods, even outperformed some supervised methods. \dd{Besides, contrastive learning is also adopted for self-supervised learning from unlabeled video \cite{timecontra} and for speaker recognition \cite{speakcontra}.} Generally, unsupervised contrastive learning has shown its great power in the computer vision field. 

To some extent, representative learning method cares about the accurate details of data, while discriminative learning method pays attention to the information in a higher level. Naturally, we hope to use the advantages of both methods in feature extraction. However, as far as we know, few contrastive learning methods have been reported in the hyperspectral classification field. There are major problems to be addressed to transfer the unsupervised contrastive learning method to the process of hyperspectral image. First, the computer vision field's typical data augmentation methods seem not reasonable in the hyperspectral classification field. For example, color distortion to the normal images will not change objects' spatial features, so it is an acceptable transformation. When distorting hyperspectral images' spectral value, the spectral information is destroyed, and the spectral information is essential for hyperspectral classification, so this is not an acceptable transformation for hyperspectral images. Second, unsupervised contrastive learning for normal images demands large batch size and lots of GPUs, because the larger the batch size is, the more information can be utilized from negative samples. However, if it is directly applied to hyperspectral images, the requirement for more computing resources will be too expensive. 


PCL showed great power of unsupervised learning in processing normal images. However, as mentioned above, it is hard to apply PCL to hyperspectral images directly. So we must make some adjustments to PCL in order to apply it to hyperspectral classification. With the blossom of AE-based methods in the hyperspectral images field, we find that the encoder in an autoencoder structure can be seen as a transformation, just like other data augmentation methods. They both map the original images from the original distribution to another distribution. The difference is, data augmentations usually do not change the shape of images, while encoder usually encodes the images to vectors with less dimensions. Another essential truth is that data augmentation methods usually keep most information of the original images to make them able to be correctly classified. Likewise, the encoder in a trained autoencoder also can keep most information in the original images.

As a result, we find it reasonable to treat the encoder as a transformation function that plays the role of data augmentation. Then the question is to find two encoders with different distributions, just like two kinds of data augmentations. So we choose designed adversarial autoencoder (AAE) and variational autoencoder (VAE) modules to act as two kinds of data augmentation because AAE and VAE can generate relatively fixed and slightly different distributions. Then the PCL only needs to learn from two kinds of vectors other than two entire images.

In this way, we can not only apply PCL to hyperspectral images but also lower the demand for deep networks, because the network for PCL only needs to process vectors with low dimensions. By encoding the images to shape fixed vectors (e.g., 1024-d), we can assign the feature extraction and contrastive learning into two parts, and each part will not be too complicated. Through this method, we make contrastive learning methods affordable for those who have limited computing resources. 

To apply the unsupervised contrastive learning to hyperspectral classification, we addressed the two problems and proposed ContrastNet, a deep learning model for unsupervised feature learning of hyperspectral images. Our innovations can be concluded as follows:
\begin{enumerate}[1)]
\item  We introduced discriminative learning methods into remote sensing field. Specifically, we applied the prototypical contrastive learning to unsupervised feature learning for hyperspectral classification.
\item Enlightened by the autoencoder structure, we \dr{introduced} two autoencoder-based modules: adversarial autoencoder module(AAE module), variational autoencoder module(VAE module). The two modules can work alone for feature extraction. When using the extracted features for hyperspectral classification, they outperformed many baselines, even supervised methods.
\item We proposed an excellent pipeline to process the hyperspectral images, which combines two kinds of unsupervised learning methods (representative learning and contrastive learning). And this pipeline shows good performance in unsupervised feature learning for hyperspectral classification. Furthermore, the pipeline only demands a single GPU, which means it is more affordable than the original prototypical contrastive learning method.

\end{enumerate}
\section{Related Work}
\subsection{Variational Autoencoder}
AE structure \cite{AE} is a widely used unsupervised feature extraction model. The standard AE is composed of an encoder and a decoder. The encoder encodes the input images to features with fixed shape. Moreover, the features are called latent code. The decoder decodes the latent code to generate forgery images similar to the input images. The AE's objective function is usually reconstruction loss(e.g., Euclidean distances between output and input). Furthermore, the whole model is optimized by the backpropagation algorithm. 

However, original AE does not restrict the distribution of latent code. Thus variational autoencoder (VAE) \cite{VAE} is proposed to optimize the distribution of latent code. VAE used KL-divergence and the reparameterization trick to restrict latent code distribution so that randomly sampled value from a normal distribution can be decoded to an image with similar distribution to the training samples. The latent code generated by VAE performs better in the classification task, so VAE is widely used for unsupervised feature extraction.
\subsection{Adversarial Autoencoder}
Adversarial autoencoder (AAE) \cite{AAE} is another AE-based structure which adopts adversarial restriction on the latent code. Unlike VAE, AAE does not use KL-divergence to measure the distance between latent code distribution and normal distribution. AAE chooses to use the idea of adversarial to restrict the distribution of latent code. By training a generative adversarial network (GAN) \cite{GAN} with the latent code and randomly selected samples from a normal distribution, the distribution of latent code will become an expected normal distribution. As a result, the latent code generated by AAE will be helpful for classification, and its distribution will be similar but different from the VAE's latent code distribution.
\subsection{Prototypical Contrastive Learning}
Usual unsupervised contrastive learning methods aim to find an embedding space where every sample can be discriminated among other instances in the whole dataset, such as momentum contrast (MoCo) \cite{Moco}. But this objective may be too hard to achieve without enough computing resources or sufficient iteration. Although this kind of distribution may be beneficial in some downstream tasks, it is not very fit for classification. Excellent distribution for classification demands for clear clusters composed of the data in the same classes. And typical unsupervised contrastive learning can't satisfy this demand.

PCL \cite{PCL} is an unsupervised representation learning method based on contrastive learning. Unlike most contrastive learning methods, PCL introduces prototypes as latent variables to help find the maximum-likelihood estimation of the network parameters in an expectation-maximization framework. PCL uses ProtoNCE loss, a generalized version of the InfoNCE \cite{InfoNCE} loss for contrastive learning by encouraging representations to be closer to their assigned prototypes. The experiments show that PCL can get better performances than other baselines in the classification tasks, so we choose PCL as our method's base structure.
\section{Proposed Method}
\subsection{VAE Module}
To process the hyperspectral images, we design a VAE network to extract features from the original hyperspectral images. The structure of the VAE module is shown in Fig.\ref{fig:VAE}. As the figure shows, we first use PCA to preprocess the whole hyperspectral image to reduce the number of the channels. Then sliding windows are adopted to split the image into small patches with the shape \dd{$s \times s \times k$}. $s$ is the size of sliding windows, and $k$ is the channel of the preprocessed hyperspectral image. The structure of the encoder network is enlightened by the idea of hybrid convolution in HybridSN \cite{HybridSN}. We used several 3D convolutional layers and 2D convolutional layers to extract the input patches' spectral and spatial information. We also used several 3D transposed convolutional layers and 2D transposed convolutional layers to build the decoder network.

Furthermore, to avoid the risk of overfitting, we adopted batch normalization \cite{bn} after every convolutional layer. Every linear layer is combined with a  rectified linear unit (ReLU) activation layer except the output layer. We use a global pooling layer to fix the shape of the feature map, thus fix the shape of extracted features (e.g., 1024-d) after reshaping operation.

According to the original VAE, we let the encoder output two variables $\mu$ and $\sigma$. Then the latent code can be computed by Eq. \ref{eqa:vae_code}. $z$ is the latent code, and $\varepsilon$ is a random value drawn from the normal distribution. The loss function for VAE network can be divided into two parts: $\mathcal{L}_{\mu, \sigma^{2}}$ and $\mathcal{L}_{recon}$. $\mathcal{L}_{\mu, \sigma^{2}}$ controls the distribution of latent code, and $\mathcal{L}_{recon}$ ensures the preservation of the input image's information. As Eq. \ref{eqa:vae_ll} shows, $N$ is the number of samples, $\mathcal{L}_{\mu, \sigma^{2}}$ computes the KL divergence between latent code and normal distribution. Moreover, Eq. \ref{eq:recon} shows the detail of reconstruction loss $\mathcal{L}_{recon}$, $N$ is the number of samples, the input image patch is $I^{x, y, z}$ with the shape of $s \times s \times k$, and $\hat{I}^{x, y, z}$ is the output image patch of the decoder. The whole loss function can be represented by Eq. \ref{eqa:vaeloss}.

\begin{figure*}
\centering
\includegraphics[width=6.5in]{VAE.pdf}
\caption{Structure of VAE module.}
\label{fig:VAE}
\end{figure*}

\begin{equation}
\label{eqa:vae_code}
{
z=\mu+\varepsilon \times \sigma
}
\end{equation}


\begin{equation}
\label{eqa:vae_ll}
{
\mathcal{L}_{\mu, \sigma^{2}}=\frac{1}{2} \sum_{i=1}^{N}\left(\mu_{(i)}^{2}+\sigma_{(i)}^{2}-\log \sigma_{(i)}^{2}-1\right)}
\end{equation}

\begin{equation}
\label{eq:recon}
\mathcal{L}_{recon}=\sum_{i=1}^{N}\left( \frac{1}{s \times s \times k} \sum_{x=0}^{s-1} \sum_{y=0}^{s-1} \sum_{z=0}^{k-1}\left(I^{x, y, z}-\hat{I}^{x, y, z}\right)^{2}\right)
\end{equation}

\begin{equation}
\label{eqa:vaeloss}
\mathcal{L}=\mathcal{L}_{\mu, \sigma^{2}}+\mathcal{L}_{recon}
\end{equation}

When we finished the VAE module training, we can map all the patches to VAE features. Thus we can use these VAE features to build the training dataset for ContrastNet.
\subsection{AAE Module}
Similar to the VAE module, the whole hyperspectral image is preprocessed by PCA in the AAE module. The structure of the AAE network is shown in Fig.\ref{fig:AAE}. The encoder and the decoder in the AAE module are the same with that in the VAE module except for the linear layers before the latent code. The encoder in the AAE module directly outputs the latent code and acts as a GAN generator.

According to the original AAE, the latent code is the output of the generator and the discriminant input. Another input of the discriminant is a randomly drawn variable from the normal distribution. The training of the AAE can be divided into two phases: reconstruction phase and regularization phase. In the reconstruction phase, we use reconstruction loss to optimize the parameters in the network. Reconstruction loss is shown in Eq. \ref{eq:recon2}, it is the same as the reconstruction loss in the VAE module. $\mathcal{L}_{recon}^{AAE}$ is reconstruction loss, its definition is the same as $\mathcal{L}_{recon}$.

In the regularization phase, the discriminator and the encoder are optimized. At first, we optimize the discriminator and then the generator (encoder). In order to stablize the training process of GAN, we adopt Wasserstein GAN (WGAN) \cite{WGAN} loss as our optimization function for the discriminator and the generator. Discriminant loss and generator loss are shown in Eq. \ref{eqa:LD} and \ref{eqa:LG}, where  $\mathcal{L}_D$ represents the loss of the discriminant, and $\mathcal{L}_G$ represents the loss of the generator. $P_{g}$ is the distribution of the generated samples(latent code), and $P_{r}$ is the distribution of the real samples(samples from a normal distribution). x represents random samples from $P_{g}$ and $P_{r}$.

\begin{figure*}
\centering
\includegraphics[width=6.5in]{AAE.pdf}

\caption{Structure of AAE module.}
\label{fig:AAE}
\end{figure*}

\begin{equation}
\label{eq:recon2}
\mathcal{L}_{recon}^{AAE}=\sum_{i=1}^{N}\left( \frac{1}{s \times s \times k} \sum_{x=0}^{s-1} \sum_{y=0}^{s-1} \sum_{z=0}^{k-1}\left(I^{x, y, z}-\hat{I}^{x, y, z}\right)^{2}\right)
\end{equation}
\begin{equation}
\label{eqa:LD}{
\mathcal{L}_D=\mathbb{E}_{x \sim P_{g}}\left[\mathbf{D}(x)\right]-\mathbb{E}_{x \sim P_{r}}\left[\mathbf{D}(x)\right]
}
\end{equation}

\begin{equation}
\label{eqa:LG}
{
\mathcal{L}_G=-\mathbb{E}_{x \sim P_{g}}\left[\mathbf{D}(x)\right]
}
\end{equation}

Similarly, when we finished the training of the AAE module, we can map all the patches to AAE features. Thus we can use these AAE features to build the training dataset for ContrastNet.

\subsection{ContrastNet}
Before we introduce the ContrastNet, the specific description of typical unsupervised contrast learning should be clarified. Let the \dd{training} set $X=\{{x_1,x_2,...,x_n}\}$ contain $n$ images. And our goal is to find an embedding function $f_\theta$(realized via a deep neural network) that maps $X$ to another space $V=\{{v_1,v_2,...,v_n}\}$ where $v_i=f_\theta(x_i)$, and $v_i$ can describe $x_i$ best. Usually the objective is achieved by the InfoNCE loss function \cite{cpc} as Eq. \ref{eq:infoNCE} shows. $v'_i$ is a positive embedding for instance $i$, and $v'_j$ includes one positive embedding (assume $v'_0=v'_i$ ) and r negative embeddings for other instances, and $\tau$ is a temperature hyper-parameter. In MoCo \cite{Moco}, these embeddings are obtained by feeding $x_i$ to a momentum encoder parametrized by $\theta'$, $v'_i=f_{\theta'}(x_i)$, where $\theta'$ is a moving average of $\theta$.


\begin{equation}
\label{eq:infoNCE}{
\mathcal{L}_{\mathrm{InfoNCE}}=\sum_{i=1}^{n}-\log \frac{\exp \left(v_{i} \cdot v_{i}^{\prime} / \tau\right)}{\sum_{j=0}^{r} \exp \left(v_{i} \cdot v_{j}^{\prime} / \tau\right)}
}
\end{equation}

When minimizing the Eq. \ref{eq:infoNCE}, the distance between $v_i$ and $v'_i$ are becoming close, and the distance between $v_i$ and $r$ negative embeddings are becoming far. However, original InfoNCE loss uses a fixed $\tau$, which means the same concentration on a certain scale. Moreover, it computes the distance between $v_i$ and all kinds of negative embeddings, some of which are not representative.




\begin{equation}
\label{eq:Proto}
\mathcal{L}_{Proto}= \sum_{i=1}^{n}-\left(\frac{1}{M} \sum_{m=1}^{M} \log \frac{\exp \left(v_{i} \cdot c_{s}^{m} / \phi_{s}^{m}\right)}{\sum_{j=0}^{r} \exp \left(v_{i} \cdot c_{j}^{m} / \phi_{j}^{m}\right)}\right)
\end{equation}

As a result, PCL proposed a new loss function named ProtoNCE. As Eq. \ref{eq:Proto} and Eq. \ref{eq:ProtoNCE} show, based on InfoNCE, ProtoNCE contains a second part $\mathcal{L}_{Proto}$. It use prototypes $c$ instead of $v'$, and replace the fixed temperature $\tau$ with a per-prototype concentration estimation $\phi$. 

\begin{equation}
\label{eq:ProtoNCE}
\mathcal{L}_{ProtoNCE}= \mathcal{L}_{Proto} +\mathcal{L}_{\mathrm{InfoNCE}} 
\end{equation}

The detailed algorithm of PCL can be found in Algorithm \ref{alg:PCL}. There are two encoders in the PCL algorithm, query encoder maps $x_i$ to $v_i$, and the momentum encoder maps $x_i$ to $v'_i$. Practically, we do not use the same $x_i$ to get $v_i$ and $v'_i$, two images with proper data augmentation will be the input of two encoders for better performance. \dd{For example, we can generate $x'_i$ by applying color distortion to $x_i$, and get $x''_i$ by applying random crop to $x_i$. Then we use $x'_i$ and $x''_i$ to get $v_i$ and $v'_i$. } The query encoder's parameters can be represented by $\theta$, and the momentum encoder's parameters can be represented by $\theta'$ which meets Eq. \ref{eq:theta}. In algorithm \ref{alg:PCL}, $k-means(\cdot,\cdot)$ \cite{faiss} is the GPU implementation of a widely used clustering algorithm. And $C^m$ is the sets of $k_m$ prototypes(center of clusters). $Concentration(\cdot,\cdot)$ is the function of concentration estimation $\phi$, as Eq. \ref{eq:phi} shows, $\phi$ is calculated by the momentum features $\{v'_z\}^Z_{z=1}$ that are within the same clusters as a prototype $c$, $\alpha$ is a smooth parameter to ensure that small clusters do not have overly-large $\phi$, and the typical value is 10. $SGD(\cdot,\cdot)$ \cite{sgd} is a kind of optimization function to update the parameters in the query encoder.


\begin{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\caption{Prototypical Contrastive Learning.}
\label{alg:PCL}
\begin{algorithmic}[1]
\Require encoder $f_\theta$, training dataset $X$, number of clusters $K=\{k_m\}^M_{m=1}$
\State $\theta'=\theta$
\While{not MaxEpoch} 

\State $V'=f_\theta'(X)$
	\For{$m = 1$ \textbf{to} $M$}
	\State $C^m=k-means(V',k_m)$
	\State $\phi^m=Concentration(C^m,V')$
	\EndFor
	\For{$x$ \textbf{in} $Dataloader(X)$}
	\State $v=f_\theta(x),v'=f'_\theta(x)$
	\State $\mathcal{L}_{ProtoNCE}(v,v',\{C^m\}^M_{m=1},\{\phi^m\}^M_{m=1})$
	\State $\theta=SGD(\mathcal{L}_{ProtoNCE},\theta)$
	\State $\theta'=0.999*\theta'+0.001*\theta$
	\EndFor
\EndWhile 
\end{algorithmic}
\end{algorithm}

\begin{equation}
\label{eq:theta}
\theta'=0.999*\theta'+0.001*\theta
\end{equation}


\begin{equation}
\label{eq:phi}
\phi=\frac{\sum_{z=1}^{Z}\left\|v_{z}^{\prime}-c\right\|_{2}}{Z \log (Z+\alpha)}
\end{equation}

The proposed ContrastNet is similar to the original PCL algorithm, but there are several differences. Firstly, ContrastNet uses AAE and VAE features as inputs, not two perturbed images. Secondly, the structure of ContrastNet is more straightforward and specialized in the "contrastive" part, not the "encoding" part. Thirdly, we adopt the projection head trick in sim-CLR \cite{simclr} to improve the performance.
\begin{figure*}
\centering
\includegraphics[width=6.5in]{ContrastNet.pdf}
\caption{
Structure of ContrastNet. Clustering means k-means algorithm, and ProtoNCE is $\mathcal{L}_{ProtoNCE}$ in Eq. \ref{eq:ProtoNCE}. M-step and E-step are the phases of Expectation-Maximization algorithm. 
}
\label{fig:ContrastNet}
\end{figure*}

Fig. \ref{fig:ContrastNet} is an overview of the ContrastNet. Expectation-Maximization (EM) algorithm is adopted to train the ContrastNet. In the E-step, VAE features are fed into the momentum encoder, then $C^m$ and $\phi^m$ are calculated. In the M-step, $\mathcal{L}_{ProtoNCE}$ is calculated based on the updated features and variables in the E-step, then the query encoder is updated via backpropagation, the momentum encoder is updated via moving average (Eq. \ref{eq:theta}).
Similarly, all convolutions in the ContrastNet are composed of a convolutional layer and a batch normalization layer, and every linear layer is combined with a ReLU layer. The 1024-d AAE and VAE features will be reshaped to $4 \times 4 \times 64$ feature maps first, in this way, the spatial information extracted can be preserved. And then, the feature maps are fed into the ContrastNet. The structure of ContrastNet is light and straightforward because the previous process has achieved the feature extraction. The ContrastNet only needs to pay attention to the contrastive learning. We adopted the projection head structure in the ContrastNet, that is, we use the output of the projection head for training, and use the features before the head for testing. Projection head acts as a nonlinear trasformation $g()$, and embedded variable $v$ is the transformation of contrast feature $z$, just as Eq. \ref{eq:projection} shows.

\begin{equation}
\label{eq:projection}
v=g(z)
\end{equation}

We use $v$ to supervise the update of ContrastNet in the training phase, and use $z$ for downstream work in the testing phase.  In this way, the extracted contrast features will contain more original information. In the testing phase, we only need the query encoder to extract contrast features in Fig. \ref{fig:ContrastNet}, thus can save much testing time for the ContrastNet.
\section{Experiments and Analysis}

To illustrate the great feature learning ability of ContrastNet, we use classification as application to validate the performance. As a simple and commonly used classifier, SVM was used for highlighting the effectiveness of the extracted features, which were learned by ContrastNet. 
Classification experiments were conducted using three publicly available HSI datasets: Indian Pines(IP), University of Pavia(PU), and Salinas Scene(SA). Eleven other methods were adopted as baselines for comparison.

They are linear discriminant analysis (LDA) \cite{LDA}, locality-preserving dimensionality reduction (LFDA) \cite{LFDA}, sparse graph-based discriminant analysis (SGDA) \cite{SGDA}, sparse and low-rank graph for discriminant analysis (SLGDA) \cite{SLGDA}, deep convolutional neural networks (1D-CNN) \cite{1D-CNN}, supervised deep feature extraction (S-CNN) \cite{S-CNN}, tensor principal component analysis (TPCA) \cite{TPCA}, stacked sparse autoencoder (SSAE) \cite{SSAE}, unsupervised deep feature extraction (EPLS) \cite{EPLS}, and 3D convolutional autoencoder (3DCAE) \cite{3DCAE}. \dd{All experiments are repeated three times, and we recorded the mean value of all results.}
\subsection{Datasets}

Experiments are conducted using three publicly available HSI datasets: Indian Pines (IP), University of Pavia (PU), and Salinas Scene (SA). The IP dataset was gathered using the Airborne Visible / Infrared Imaging Spectrometer (AVIRIS)  hyperspectral sensor. It consisted of 145$\times$145 pixels and 224 spectral reflectance bands in the wavelength range of $0.4\sim2.5 \times10^{-6}$ meters. After removing bands covering the region of water absorption, 200 bands were left, and the ground truth was composed of 16 classes. In this dataset, there is a serious problem of uneven sample size. The class with the largest number of samples has more than two thousand samples, while the class with the smaller number of samples has only 20 samples. The details of the IP dataset are shown in Table \ref{tab:data_IP}.

\begin{table}
\caption{Details of the IP dataset. }
\label{tab:data_IP}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
\multicolumn{3}{|c|}{IP Dataset}                                                                                      \\ \hline
Class Name                      & Index                        & Number                            \\ \hline
Alfalfa                         & 0                            & 46                                                   \\ \hline
Corn-notill                     & 1                            & 1428                                                 \\ \hline
Corn-mintill                    & 2                            & 830                                                 \\ \hline
Corn                            & 3                            & 237                                                  \\ \hline
Grass-pasture                   & 4                            & 483                                                  \\ \hline
Grass-trees                     & 5                            & 730                                                  \\ \hline
Grass-pasture-mowed             & 6                            & 28                                                   \\ \hline
Hay-windrowed                   & 7                            & 478                                                  \\ \hline
Oats                            & 8                           & 20                                                   \\ \hline
Soybean-notill                  & 9                           & 972                                                  \\ \hline
Soybean-mintill                 & 10                            & 2455                                                 \\ \hline
Soybean-clean                   & 11                            & 593                                                  \\ \hline
Wheat                           & 12                            & 205                                                  \\ \hline
Woods                           & 13                            & 1265                                                 \\ \hline
Buildings-Grass-Trees-Drives    & 14                           & 386                                                  \\ \hline
Stone-Steel-Towers              & 15                            & 93                                                   \\ \hline
\textbf{Total} &    & \multicolumn{1}{c|}{\textbf{10249}} \\ \hline
\end{tabular}
\end{center}
\end{table}




The PU dataset was a hyperspectral image with 610$\times$340 pixels and 103 spectral bands in the wavelength range of $0.43\sim0.86 \times10^{-6}$ meters. The ground truth contained nine classes. The characteristics of this dataset are that the background pixels are complex, the area of the connected region is small, and there are many discontinuous pixels. The details of the PU dataset are shown in Table \ref{tab:data_PU}.


\begin{table}
\caption{Details of the PU dataset. }
\label{tab:data_PU}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
\multicolumn{3}{|c|}{UP Dataset}                    \\ \hline
Class Name           & Index       & Number           \\ \hline
Asphalt              & 0           & 6631           \\ \hline
Meadows              & 1           & 18649          \\ \hline
Gravel               & 2           & 2099           \\ \hline
Trees                & 3           & 3064           \\ \hline
Painted metal sheets & 4           & 1345           \\ \hline
Bare Soil            & 5           & 5029           \\ \hline
Bitumen              & 6           & 1330           \\ \hline
Self-Blocking Bricks & 7           & 3682           \\ \hline
Shadows              & 8           & 947            \\ \hline
\textbf{Total}       &   & \textbf{42776} \\ \hline
\end{tabular}
\end{center}
\end{table}

The SA dataset was an image with 512$\times$217 pixels and 224 spectral bands. This dataset was in the wavelength range of $0.36\sim2.5 \times10^{-6}$ meters. Twenty water-absorbing bands were discarded from the SA dataset, so it was a dataset with 204 spectral bands and 16 landcover classes in the ground truth. The background pixels of this dataset are not complex, and there is no problem of uneven number of samples. Compared with the other two datasets, it is easier to classify. The details of the SA dataset are shown in Table \ref{tab:data_SA}.
\begin{table}
\caption{Details of the SA dataset.  }
\label{tab:data_SA}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
\multicolumn{3}{|c|}{SA Dataset}                            \\ \hline
Class Name                   & Index       & Number           \\ \hline
Brocoli\_green\_weeds\_1     & 0           & 2009           \\ \hline
Brocoli\_green\_weeds\_2     & 1           & 3726           \\ \hline
Fallow                       & 2           & 1976           \\ \hline
Fallow\_rough\_plow          & 3           & 1394           \\ \hline
Fallow\_smooth               & 4           & 2678           \\ \hline
Stubble                      & 5           & 3959           \\ \hline
Celery                       & 6           & 3579           \\ \hline
Grapes\_untrained            & 7           & 11271          \\ \hline
Soil\_vinyard\_develop       & 8           & 6203           \\ \hline
Corn\_senesced\_green\_weeds & 9           & 3278           \\ \hline
Lettuce\_romaine\_4wk        & 10          & 1068           \\ \hline
Lettuce\_romaine\_5wk        & 11           & 1927           \\ \hline
Lettuce\_romaine\_6wk        & 12           & 916            \\ \hline
Lettuce\_romaine\_7wk        & 13           & 1070           \\ \hline
Vinyard\_untrained           & 14           & 7268           \\ \hline
Vinyard\_vertical\_trellis   & 15           & 1807           \\ \hline
\textbf{Total}               &   & \textbf{54129} \\ \hline
\end{tabular}
\end{center}
\end{table}
\subsection{Parameters Setting}
\subsubsection{Training sample and testing sample selection}
10\% samples of each class are randomly selected for training SVM in the Indian Pines and University of Pavia datasets, and 5\% samples of each class are used for training in the Salinas dataset, the rest in each dataset is used for testing.

\subsubsection{Parameters in model}
All experiments were implemented on a PC with 16GB RAM and a GTX 1080 GPU. The coding environment was pytorch \cite{pytorch}. The shape of patches is $27 \times 27 \times 15$ in PU and SA dataset, and $27 \times 27 \times 30$ in the IP dataset. When we use $27 \times 27 \times 15$ patches, our networks' details are shown as follows.

Table \ref{tab:AAE_enc} and Table \ref{tab:AAE_dec} show the structure of AAE. The structure of the discriminant is simple, so it is omitted. The latent code dimension is 128 and extracted AAE features are flattened outputs of the pooling layer in the encoder(1024-d). In the training phase, we use two Adam \cite{adam} optimizers to optimize the encoder and the decoder, and two SGD \cite{sgd} optimizers to optimize the generator and the discriminant. Two Adam optimizers are set with the learning rate of 0.001, and weight decay is set to 0.0005. The optimizer for the generator is set with a 0.0001 learning rate and no weight decay. The optimizer for the discriminant is set with a 0.00005 learning rate and no weight decay. The batch size is set to 128. We train the AAE module for 20 epochs, and only save the parameters of the encoder.
\begin{table}
\caption{Structure of AAE Encoder. The shape of data is defined in pytorch style. -1 means batchsize in the shape array.}
\label{tab:AAE_enc}

\centering
\begin{tabular}{|c|c|}
\hline
\multicolumn{2}{|c|}{AAE Encoder}       \\ \hline
Layer(type)       & Output Shape        \\ \hline
input             & {[}-1,1,15,27,27{]} \\ \hline
Conv3d            & {[}-1,8,9,25,25{]}  \\ \hline
BatchNorm3d       & {[}-1,8,9,25,25{]}  \\ \hline
ReLU              & {[}-1,8,9,25,25{]}  \\ \hline
Conv3d            & {[}-1,16,5,23,23{]} \\ \hline
BatchNorm3d       & {[}-1,16,5,23,23{]} \\ \hline
ReLU              & {[}-1,16,5,23,23{]} \\ \hline
Conv3d            & {[}-1,32,3,21,21{]} \\ \hline
BatchNorm3d       & {[}-1,32,3,21,21{]} \\ \hline
ReLU              & {[}-1,32,3,21,21{]} \\ \hline
Conv2d            & {[}-1,64,19,19{]}   \\ \hline
BatchNorm2d       & {[}-1,64,19,19{]}   \\ \hline
ReLU              & {[}-1,64,19,19{]}   \\ \hline
AdaptiveAvgPool2d & {[}-1,64,4,4{]}     \\ \hline
Linear            & {[}-1,512{]}        \\ \hline
ReLU              & {[}-1,512{]}        \\ \hline
Linear            & {[}-1,128{]}        \\ \hline
\end{tabular}
\end{table}

\begin{table}
\caption{Structure of AAE Decoder. The shape of data is defined in pytorch style. -1 means batchsize in the shape array.}
\label{tab:AAE_dec}
\centering
\begin{tabular}{|c|c|}
\hline
\multicolumn{2}{|c|}{AAE Decoder}      \\ \hline
Layer(type)      & Output Shape        \\ \hline
input            & {[}-1,128{]}        \\ \hline
Linear           & {[}-1,256{]}        \\ \hline
ReLU             & {[}-1,256{]}        \\ \hline
Linear           & {[}-1,23104{]}      \\ \hline
ReLU             & {[}-1,23104{]}      \\ \hline
ConvTransposed2d & {[}-1,96,21,21{]}   \\ \hline
BatchNorm2d      & {[}-1,96,21,21{]}   \\ \hline
ReLU             & {[}-1,96,21,21{]}   \\ \hline
ConvTransposed3d & {[}-1,16,5,23,23{]} \\ \hline
BatchNorm3d      & {[}-1,16,5,23,23{]} \\ \hline
ReLU             & {[}-1,16,5,23,23{]} \\ \hline
ConvTransposed3d & {[}-1,8,9,25,25{]}  \\ \hline
BatchNorm3d      & {[}-1,8,9,25,25{]}  \\ \hline
ReLU             & {[}-1,8,9,25,25{]}  \\ \hline
ConvTransposed3d & {[}-1,1,15,27,27{]} \\ \hline
BatchNorm3d      & {[}-1,1,15,27,27{]} \\ \hline
\end{tabular}
\end{table}

Table \ref{tab:VAE_enc} and Table \ref{tab:VAE_dec} show the structure of VAE. The dimension of latent code is also 128 and extracted VAE features are flattened outputs of the pooling layer in the encoder(1024-d) too. In the training phase, we use two Adam \cite{adam} optimizers to optimize the encoder and the decoder. Two Adam optimizers are set with the learning rate of 0.001, and weight decay is set to 0.0005. The two outputs of VAE encoder are used to compute the latent code. Then the latent code is fed into the decoder. The batch size is set to 128. We train the VAE module for 30 epochs, and only save the parameters of the encoder.

\begin{table}
\caption{Structure of VAE Encoder. The shape of data is defined in pytorch style. -1 means batchsize in the shape array.}
\label{tab:VAE_enc}
\centering
\begin{tabular}{|c|c|}
\hline
\multicolumn{2}{|c|}{VAE Encoder}             \\ \hline
input             & {[}-1,1,15,27,27{]}       \\ \hline
Conv3d            & {[}-1,8,9,25,25{]}        \\ \hline
BatchNorm3d       & {[}-1,8,9,25,25{]}        \\ \hline
ReLU              & {[}-1,8,9,25,25{]}        \\ \hline
Conv3d            & {[}-1,16,5,23,23{]}       \\ \hline
BatchNorm3d       & {[}-1,16,5,23,23{]}       \\ \hline
ReLU              & {[}-1,16,5,23,23{]}       \\ \hline
Conv3d            & {[}-1,32,3,21,21{]}       \\ \hline
BatchNorm3d       & {[}-1,32,3,21,21{]}       \\ \hline
ReLU              & {[}-1,32,3,21,21{]}       \\ \hline
Conv2d            & {[}-1,64,19,19{]}         \\ \hline
BatchNorm2d       & {[}-1,64,19,19{]}         \\ \hline
ReLU              & {[}-1,64,19,19{]}         \\ \hline
AdaptiveAvgPool2d & {[}-1,64,4,4{]}           \\ \hline
Linear            & {[}-1,512{]}              \\ \hline
ReLU              & {[}-1,512{]}              \\ \hline
Linear/Linear     & {[}-1,128{]}/{[}-1,128{]} \\ \hline
\end{tabular}
\end{table}

\begin{table}
\caption{Structure of VAE Decoder. The shape of data is defined in pytorch style. -1 means batchsize in the shape array.}
\label{tab:VAE_dec}
\centering
\begin{tabular}{|c|c|}
\hline
\multicolumn{2}{|c|}{VAE Decoder}      \\ \hline
Layer(type)      & Output Shape        \\ \hline
input            & {[}-1,128{]}        \\ \hline
Linear           & {[}-1,256{]}        \\ \hline
ReLU             & {[}-1,256{]}        \\ \hline
Linear           & {[}-1,23104{]}      \\ \hline
ReLU             & {[}-1,23104{]}      \\ \hline
ConvTransposed2d & {[}-1,96,21,21{]}   \\ \hline
BatchNorm2d      & {[}-1,96,21,21{]}   \\ \hline
ReLU             & {[}-1,96,21,21{]}   \\ \hline
ConvTransposed3d & {[}-1,16,5,23,23{]} \\ \hline
BatchNorm3d      & {[}-1,16,5,23,23{]} \\ \hline
ReLU             & {[}-1,16,5,23,23{]} \\ \hline
ConvTransposed3d & {[}-1,8,9,25,25{]}  \\ \hline
BatchNorm3d      & {[}-1,8,9,25,25{]}  \\ \hline
ReLU             & {[}-1,8,9,25,25{]}  \\ \hline
ConvTransposed3d & {[}-1,1,15,27,27{]} \\ \hline
BatchNorm3d      & {[}-1,1,15,27,27{]} \\ \hline
\end{tabular}
\end{table}

The two encoders in ContrastNet have the same structure, which is shown in Table \ref{tab:Contrast_enc}. Two inputs are 1024-d vectors, and the dimension of contrast features and projected features are both 128-d. We train the ContrastNet with an SGD optimizer, and the learning rate is 0.003, weight decay is set to 0.001. Number of negative samples $r=640$, and batch size is 128, $\tau$ in Eq. \ref{eq:infoNCE} is 0.01, number of clusters $K=[1000,1500,2500]$. According to the original PCL method, we only train the network with Eq. \ref{eq:infoNCE} for 30 epochs, then train the network with Eq. \ref{eq:ProtoNCE} for 170 epochs. The learning rate will be multiplied with 0.1 when the trained epoch is more than 120 and 160.



\begin{table}
\caption{Structure of ContrastNet Encoder. The shape of data is defined in pytorch style. -1 means batchsize in the shape array.}
\label{tab:Contrast_enc}
\centering
\begin{tabular}{|c|c|}
\hline
\multicolumn{2}{|c|}{ContrastNet Encoder} \\ \hline
Layer(type)         & Output Shape        \\ \hline
input               & {[}-1,1024{]}       \\ \hline
ConvTransposed2d    & {[}-1,64,6,6{]}     \\ \hline
BatchNorm2d         & {[}-1,64,6,6{]}     \\ \hline
ReLU                & {[}-1,64,6,6{]}     \\ \hline
ConvTransposed2d    & {[}-1,64,8,8{]}     \\ \hline
BatchNorm2d         & {[}-1,64,8,8{]}     \\ \hline
ReLU                & {[}-1,64,8,8{]}     \\ \hline
Conv2d              & {[}-1,128,6,6{]}    \\ \hline
BatchNorm2d         & {[}-1,128,6,6{]}    \\ \hline
ReLU                & {[}-1,128,6,6{]}    \\ \hline
Conv2d              & {[}-1,64,4,4{]}     \\ \hline
BatchNorm2d         & {[}-1,64,4,4{]}     \\ \hline
ReLU                & {[}-1,64,4,4{]}     \\ \hline
Conv2d              & {[}-1,32,2,2{]}     \\ \hline
ReLU                & {[}-1,32,2,2{]}     \\ \hline
Linear              & {[}-1,128{]}        \\ \hline
ReLU                & {[}-1,128{]}        \\ \hline
Linear              & {[}-1,128{]}        \\ \hline
\end{tabular}
\end{table}

\subsection{Criteria}
The quantitative results are evaluated by overall accuracy (OA) and average accuracy (AA). 

As Eq. \ref{eqa:OA} shows, overall accuracy is represented as $\mathbf{S}_{OA}$, $N_{correct}$ means the sum of samples that are classified correctly, and $N_{total}$ means all labeled samples. When applied to binary classification, $\mathbf{S}_{OA}$ means accuracy. $\mathbf{S}_{OA}$ ranges from 0 to 1, and the bigger the $\mathbf{S}_{OA}$ is, the better the classifier is. $\mathbf{S}_{OA}$ treats different classes by weighting the amount of data in each class, but it tends to be dominated by classes that contain more samples than other classes. 

\begin{equation}
\label{eqa:OA}
\mathbf{S}_{OA}=\frac{N_{correct}}{N_{total}}
\end{equation}




Eq. \ref{eqa:AA} is the definition of average accuracy, $\mathbf{S}_{AA}$ means average accuracy, $n$ is the number of classes, $\text {accuracy}_{i}$ is the classification accuracy of $\mathbf{i}$th class($i \leq n$). Similar to $\mathbf{S}_{OA}$, $\mathbf{S}_{AA}$ also ranges from 0 to 1, and it is also expected to be close to 1. However, when there are some classes with few samples, the statistical variable deviation of accuracies of these classes will be high, thus leading to distortion of the average accuracy.

\begin{equation}
\label{eqa:AA}
\mathbf{S}_{AA}=\frac{\sum\limits_{i=1}^n \text {accuracy}_{i}}{n}
\end{equation}

\subsection{Results and Analysis}
\subsubsection{Classification Experiments}
The results in the Indian Pines dataset are shown in Table \ref{tab:IP}. It is clear that the proposed structures performed best in many classes. AAE got the best results in five classes while ContrastNet got the best results in six classes, and VAE performed best in 3 classes.

To some extent, AAE and VAE are two better feature extractors than 3DCAE in term of AA, and AAE is better than VAE in both AA and OA. However, VAE shows great ability in extracting features from the classes with few numbers, such as class 0, 6, 8 and 15. The number of samples in these classes are less than 100, while other classes may have over a thousand samples. In these classes, VAE performs better than AAE, though in other classes it is not as well as AAE is. As for ContrastNet, it shows a significant increase in OA than AAE and VAE, thus outperform all methods. This can be an evidence indicating that ContrastNet can extract some core information from two distributions by contrastive learning. However, ContrastNet did not perform well enough in AA in the Indian Pines dataset. According to the table, the accuracy of ContrastNet are lower than AAE's and VAE's in class 0, 3, 5, 6, 7, 8, 12, 14, 15. And this problem is severe in the classes containing few samples, such as class 0, 6, 8 and 15. We guess the reason for it may be the imbalance of the number of samples in the Indian Pines dataset. Classes with large numbers dominated the location of clusters. Thus the ContrastNet tended to perform well in these classes, which decreased accuracy in other classes. However, ContrastNet still shows the best OA, and its AA is very close to 3DCAE, which outperforms other baselines. In other words, ContrastNet makes a trade-off between AA and OA. It tends to increase OA at the expense of lowering AA. As a result, ContrastNet gets the best OA and relatively good AA in the IP dataset.

Generally speaking, the AAE and VAE modules we designed show excellent ability in extracting features unsupervisely, and VAE is better at extracting information from classes with a small sample size. The ContrastNet we proposed utilized the features generated by AAE and VAE, further improved the ability of extracting features. However, limited by the clustering idea it introduces, it improves the OA while reducing the focus on the few sample classes, thus leading to a decline in AA.


\begin{table*}
\caption{Comparison in the Indian Pines dataset. 10\% labeled samples are used for training, and the rest are used for testing. AA menas average accuracy and OA means overall accuracy. The best values in each row are in bold. And the methods in bold are structures proposed in this paper. Some of the data in the table is quoted from \cite{3DCAE}. }
\label{tab:IP}
\scalebox{0.8}{
\begin{tabular}{c|cccccc|cccccccc}
\hline
\multirow{2}{*}{Class} & \multicolumn{6}{c|}{Supervised Feature Extraction}      & \multicolumn{8}{c}{Unsupervised Feature Extraction}                                                                    \\ \cline{2-15} 
                       & LDA   & LFDA  & SGDA  & SLGDA          & 1D-CNN & S-CNN & PCA   & TPCA            & SSAE            & EPLS  & 3DCAE          & \textbf{AAE}             & \textbf{VAE}             & \textbf{ContrastNet}       \\ \hline
0                      & 58.54 & 29.63 & 42.59 & 39.62          & 43.33  & 83.33 & 39.02 & 60.97           & 56.25           & 58.72 & 90.48          & \textbf{100.00} & \textbf{100.00} & 85.37          \\ \hline
1                      & 69.88 & 75.59 & 80.89 & 85.56          & 73.13  & 81.41 & 72.30 & 87.00           & 69.58           & 59.91 & 92.49          & 81.63           & 78.78           & \textbf{97.15} \\ \hline
2                      & 65.86 & 75.42 & 65.71 & 74.82          & 65.52  & 74.02 & 72.02 & 94.51           & 75.36           & 71.34 & 90.37          & 95.27           & 92.37           & \textbf{97.95} \\ \hline
3                      & 73.71 & 58.12 & 64.10 & 49.32          & 51.31  & 71.49 & 55.87 & 79.34           & 64.58           & 74.31 & 86.90          & \textbf{99.22}  & 97.34           & 95.62          \\ \hline
4                      & 90.32 & 95.17 & 94.57 & 95.35          & 87.70  & 90.11 & 93.09 & 93.08           & 88.81           & 97.95 & 94.25          & 95.17           & 93.87           & \textbf{96.09} \\ \hline
5                      & 92.09 & 96.12 & 98.39 & 95.59          & 95.10  & 94.06 & 94.67 & 96.34           & 87.00           & 96.44 & 97.07          & \textbf{98.73}  & 98.27           & 96.80          \\ \hline
6                      & 96.00 & 11.53 & 50.00 & 36.92          & 56.92  & 84.61 & 80.00 & 76.00           & 90.00           & 54.02 & 91.26          & 96.00           & \textbf{98.67}  & 70.67          \\ \hline
7                      & 98.14 & 93.87 & 99.80 & 99.75          & 96.64  & 98.37 & 98.37 & 99.76           & 89.72           & 88.99 & 97.79          & \textbf{99.84}  & 99.77           & 98.68          \\ \hline
8                      & 11.11 & 0.00  & 0.00  & 5.00           & 28.89  & 33.33 & 88.89 & \textbf{100.00} & \textbf{100.00} & 58.89 & 75.91          & 96.30           & 98.15           & 70.37          \\ \hline
9                     & 73.80 & 80.89 & 59.30 & 69.11          & 75.12  & 86.05 & 74.49 & 79.51           & 77.19           & 73.10 & 87.34          & 87.01           & 78.86           & \textbf{97.45} \\ \hline
10                     & 55.41 & 83.02 & 84.44 & 89.91          & 83.49  & 82.98 & 69.58 & 85.42           & 77.58           & 70.78 & 90.24          & 89.08           & 81.75           & \textbf{98.40} \\ \hline
11                     & 76.92 & 86.32 & 77.04 & 86.78          & 67.55  & 73.40 & 65.29 & 84.24           & 72.00           & 57.51 & \textbf{95.76} & 93.51           & 90.64           & 93.57          \\ \hline
12                     & 91.30 & 79.25 & 99.09 & \textbf{99.51} & 96.86  & 87.02 & 98.37 & 98.91           & 87.80           & 99.25 & 97.49          & 98.56           & 98.56           & 95.32          \\ \hline
13                     & 93.32 & 88.87 & 92.50 & 96.45          & 96.51  & 94.38 & 91.39 & 98.06           & 93.48           & 95.07 & 96.03          & 95.73           & 93.24           & \textbf{98.51} \\ \hline
14                     & 67.72 & 60.00 & 68.68 & 61.79          & 39.08  & 75.57 & 48.99 & 87.31           & 72.36           & 91.26 & 90.48          & \textbf{97.31}  & 97.02           & 96.73          \\ \hline
15                     & 90.36 & 53.68 & 85.26 & 84.16          & 89.40  & 79.76 & 87.95 & 96.38           & 97.22           & 91.27 & 98.82          & 98.02           & \textbf{98.81}  & 79.76          \\ \hline
\textbf{AA(\%)}        & 76.89 & 66.72 & 72.65 & 73.10          & 71.66  & 84.44 & 76.89 & 89.31           & 81.18           & 77.43 & 92.04          & \textbf{95.09}  & 93.51           & 91.78          \\ \hline
\textbf{OA(\%)}        & 76.88 & 81.79 & 80.05 & 85.19          & 79.66  & 80.72 & 76.88 & 88.55           & 79.78           & 77.18 & 92.35          & 91.80           & 88.03           & \textbf{97.08} \\ \hline
\end{tabular}}
\end{table*}

The results in the SA dataset are shown in Table \ref{tab:SA}. Similar to the IP dataset results, AAE performed best in five classes, VAE and ContrastNet both performed best in three classes. Since the background of the dataset is simple and there is no problem of sample size imbalance, many methods perform well on this dataset. AAE and VAE still get higher AA than other baselines, which indicates their great feature extraction ability. However, there are some methods outperform AAE and VAE in OA. S-CNN, TPCA, 3DCAE get higher OA than VAE, and S-CNN also gets higher OA than AAE. For VAE, it basically shows similar performance to AAE except in class 7 and 14. The two classes have 11271 and 7268 samples respectively, while other classes basically have less than 5000 samples. It seems the performance of VAE will be affected by the ratio of the number of samples between each class. According to the AA and OA, the performance of VAE is close to 3DCAE. For AAE, it has less OA than S-CNN but close, it is still an efficient feature extraction method. In this simpler dataset, AAE and VAE also keep relatively better performances than many methods, and this show their good generalization ability.

Though all methods got good performances in this dataset, ContrastNet still got the highest OA and got the highest AA. Unlike the IP dataset, the number of samples in the SA dataset is relatively balanced, so ContrastNet got a higher AA than AAE and VAE, and there is no obvious decrease of accuracy in each class. On the contrary, the accuracy of several classes has been significantly improved after combining the characteristics of AAE and VAE, such as class 7 and 14. There are two reasons for this phenomenon. On the one hand, ContrastNet has utilized the information shared by AAE and VAE. On the other hand, the sample size of these two classes is relatively large, thus may contain more cluster centers. Thanks to the introduction of clustering ideas, ContrastNet is easier to extract features from such classes. As a result, ContrastNet outperforms all methods in AA and OA.

\begin{table*}
\caption{Comparison in the Salinas dataset. 5\% labeled samples are used for training, and the rest are used for testing. AA menas average accuracy and OA means overall accuracy. The best values in each row are in bold. And the methods in bold are structures proposed in this paper. Some of the data in the table is quoted from \cite{3DCAE}.}
\label{tab:SA}
\scalebox{0.8}{
\begin{tabular}{c|cccccc|cccccccc}
\hline
Class  & \multicolumn{6}{c|}{Supervised Feature Extraction}                          & \multicolumn{8}{c}{Unsupervised Feature Extraction}                                                                     \\ \hline
       & LDA            & LFDA  & SGDA            & SLGDA           & 1D-CNN & S-CNN & PCA   & TPCA            & SSAE            & EPLS  & 3DCAE           & \textbf{AAE}             & \textbf{VAE}             & \textbf{ContrastNet}    \\ \hline
0      & 99.16          & 99.20 & 99.65           & 98.14           & 97.98  & 99.55 & 97.48 & 99.88           & \textbf{100.00} & 99.99 & \textbf{100.00} & 99.98           & 99.74           & 99.93          \\ \hline
1      & 99.94          & 99.19 & 99.33           & 99.44           & 99.25  & 99.43 & 99.52 & 99.49           & 99.52           & 99.92 & 99.29           & \textbf{100.00} & 99.79           & 99.80          \\ \hline
2      & 99.79          & 99.75 & 99.30           & 99.29           & 94.43  & 98.81 & 99.41 & 99.04           & 94.24           & 98.75 & 97.13           & \textbf{100.00} & \textbf{100.00} & 99.95          \\ \hline
3      & 99.77          & 99.71 & 99.21           & 99.57           & 99.42  & 97.45 & 99.77 & \textbf{99.84}  & 99.17           & 98.52 & 97.91           & 99.09           & 99.57           & 98.01          \\ \hline
4      & 98.98          & 98.47 & 99.07           & 98.06           & 96.60  & 97.96 & 98.70 & 98.96           & 98.82           & 98.33 & 98.26           & 99.42           & \textbf{99.71}  & 99.48          \\ \hline
5      & 99.89          & 99.09 & 99.57           & 99.32           & 99.51  & 99.83 & 99.65 & 99.80           & \textbf{100.00} & 99.92 & 99.98           & 99.97           & 99.86           & 99.94          \\ \hline
6      & \textbf{99.97} & 99.66 & 99.27           & 99.33           & 99.27  & 99.59 & 99.94 & 99.84           & 99.94           & 97.69 & 99.64           & 99.93           & 99.96           & 99.79          \\ \hline
7      & 81.84          & 86.89 & 89.78           & 89.48           & 86.79  & 94.40 & 83.90 & 84.11           & 80.73           & 78.86 & 91.58           & 91.21           & 86.91           & \textbf{99.53} \\ \hline
8      & 99.90          & 97.34 & \textbf{100.00} & 99.65           & 99.08  & 98.85 & 99.97 & 99.60           & 99.47           & 99.54 & 99.28           & 99.69           & 99.99           & 99.71          \\ \hline
9     & 96.31          & 95.85 & 97.99           & 97.94           & 93.71  & 97.35 & 96.89 & 95.76           & 92.12           & 95.98 & 96.65           & 98.46           & 96.54           & \textbf{99.80} \\ \hline
10     & 99.61          & 97.94 & 99.53           & 99.06           & 94.55  & 97.71 & 96.84 & 96.14           & 96.62           & 98.60 & 97.74           & 99.57           & \textbf{100.00} & 99.80          \\ \hline
11     & 99.67          & 99.64 & \textbf{100.00} & \textbf{100.00} & 99.59  & 98.73 & 99.95 & 99.07           & 97.75           & 99.44 & 98.84           & \textbf{100.00} & 99.44           & 99.98          \\ \hline
12     & 99.20          & 97.38 & 98.47           & 97.82           & 97.50  & 96.72 & 99.54 & \textbf{100.00} & 95.81           & 98.85 & 99.26           & 99.89           & 97.24           & 98.20          \\ \hline
13     & 96.56          & 93.18 & 96.07           & 90.47           & 94.08  & 95.22 & 97.24 & 95.74           & 96.65           & 98.56 & 97.49           & \textbf{99.08}  & 96.49           & 98.62          \\ \hline
14     & 73.60          & 63.04 & 65.40           & 69.51           & 66.52  & 95.61 & 76.68 & 79.54           & 79.73           & 83.13 & 87.85           & 93.69           & 87.90           & \textbf{99.53} \\ \hline
15     & 98.48          & 99.00 & 99.34           & 99.00           & 97.48  & 99.44 & 97.90 & 98.40           & 99.12           & 99.50 & 98.34           & \textbf{99.73}  & 99.61           & 99.57          \\ \hline
AA(\%) & 96.42          & 95.33 & 96.37           & 96.01           & 94.73  & 97.39 & 96.46 & 93.24           & 95.61           & 96.55 & 97.45           & 98.73           & 97.67           & \textbf{99.48} \\ \hline
OA(\%) & 92.18          & 91.22 & 91.82           & 93.31           & 91.30  & 97.92 & 92.87 & 96.57           & 92.11           & 92.35 & 95.81           & 97.10           & 95.23           & \textbf{99.60} \\ \hline
\end{tabular}}
\end{table*}



Experiment results in the PU dataset are shown in Table \ref{tab:PU}. Similarly, VAE shows a relatively good performance and AAE outperforms all baselines in AA and OA. VAE shows a surprisingly low accuracy in class 0, this may caused by the comlex background of the PU dataset. Class 0 in the PU dataset is asphalt, and it is often distributed in elongated connected areas, which makes the pixels around the center pixels more complicated, and it is difficult for VAE to encode such patches efficiently. However, AAE still performs well on such a complex dataset, especially in class 6. 

Although the background is complex, ContrastNet still outperforms all methods in this dataset.   
In the PU dataset, because of the use of the characteristics of AAE and VAE for contrastive learning, ContrastNet's accuracy on most classes surpasses AAE and VAE. Furthermore, it surpasses all methods in class 0, 1, 2 and 7. This result shows great power of ContrastNet in feature learning.


\begin{table*}
\caption{Comparison in the University of Pavia dataset. 10\% labeled samples are used for training, and the rest are used for testing. AA menas average accuracy and OA means overall accuracy. The best values in each row are in bold. And the methods in bold are structures proposed in this paper. Some of the data in the table is quoted from \cite{3DCAE}.}
\label{tab:PU}
\scalebox{0.8}{
\begin{tabular}{c|cccccc|cccccccc}
\hline
Class  & \multicolumn{6}{c|}{Supervised Feature Extraction}       & \multicolumn{8}{c}{Unsupervised Feature Extraction}                                                                             \\ \hline
       & LDA             & LFDA  & SGDA  & SLGDA & 1D-CNN & S-CNN & PCA             & TPCA            & SSAE            & EPLS           & 3DCAE  & \textbf{AAE}             & \textbf{VAE}             & \textbf{ContrastNet}    \\ \hline
0      & 78.41           & 93.45 & 91.37 & 94.66 & 90.93  & 95.40 & 90.89           & 96.17           & 95.72           & 95.95          & 95.21 & 95.39           & 81.31          & \textbf{99.49} \\ \hline
1      & 83.69           & 97.36 & 97.23 & 97.83 & 96.94  & 97.31 & 93.27           & 97.95           & 94.13           & 95.91          & 96.06 & 98.96           & 97.65          & \textbf{99.98} \\ \hline
2      & 73.02           & 71.41 & 66.08 & 77.27 & 69.43  & 81.21 & 82.60           & 86.50           & 87.47           & 94.33          & 91.32 & 97.49           & 91.00          & \textbf{99.06} \\ \hline
3      & 93.68           & 91.00 & 91.19 & 93.18 & 90.32  & 95.83 & 92.41           & 94.84           & 96.91           & \textbf{99.28} & 98.28 & 96.94           & 94.79          & 97.75          \\ \hline
4      & \textbf{100.00} & 97.99 & 99.33 & 98.51 & 99.44  & 99.91 & 98.98           & \textbf{100.00} & 99.76           & 99.92          & 95.55 & 99.94           & 99.94          & 99.81          \\ \hline
5      & 88.51           & 87.55 & 80.31 & 90.08 & 73.69  & 95.29 & 92.00           & 94.76           & 95.76           & 93.57          & 95.30 & 99.29           & \textbf{99.91} & 99.90          \\ \hline
6      & 85.75           & 80.23 & 75.26 & 85.34 & 83.42  & 87.05 & 85.83           & 91.89           & 91.18           & 98.17          & 95.14 & \textbf{100.00} & 99.42          & 99.83          \\ \hline
7      & 74.49           & 86.98 & 84.11 & 90.49 & 83.65  & 87.35 & 82.96           & 89.04           & 82.47           & 91.23          & 91.38 & 97.90           & 94.77          & \textbf{98.79} \\ \hline
8      & 99.11           & 99.26 & 95.14 & 99.37 & 98.23  & 95.66 & \textbf{100.00} & 98.94           & \textbf{100.00} & 99.78          & 99.96 & 96.32           & 88.62          & 94.84          \\ \hline
AA(\%) & 86.29           & 89.47 & 86.67 & 91.86 & 87.34  & 94.75 & 90.99           & 95.64           & 93.71           & 96.33          & 95.36 & 98.03           & 94.16          & \textbf{98.83} \\ \hline
OA(\%) & 83.75           & 92.77 & 90.58 & 94.15 & 89.99  & 92.78 & 91.37           & 94.45           & 93.51           & 95.13          & 95.39 & 98.14           & 94.53          & \textbf{99.46} \\ \hline
\end{tabular}}
\end{table*}


Generally speaking, the proposed AAE, VAE, and ContrastNet in this paper are good models that outperform many supervised and unsupervised methods. 

\dd{At first glance, it seems counterintuitive that unsupervised methods can surpass supervised methods. However, as far as this experiment is concerned, all methods have the same number of labels, and the accuracy of classification majorly depends on feature extraction. The supervised method directly uses the label information and the backpropagation algorithm to extract features (10\% or fewer samples are used), while the unsupervised method extracts the features based on the characteristics of the data itself (all samples are used). In terms of the sample size used when extracting features, unsupervised methods are much larger than supervised methods. Therefore, using unsupervised methods for feature learning is easier to learn representative and robust generalization features.

In contrast, the features learned by supervised methods are more susceptible to the difference between the distribution of labeled samples and the distribution of the real world. Moreover, using different network structures for feature learning will have different learning efficiency. Therefore, unsupervised feature learning may surpass supervised methods in feature extraction.}

Among the three methods, autoencoder-based AAE and VAE are models that make use of reconstruction information and concentrate on the single sample itself. ContrastNet is a model that learns the similarity between two different distributions of a single sample, and also learn the dissimilarity between positive samples and negative samples. According to the experiment results, AAE is a better feature extraction method than VAE under most circumstances; VAE shows potential in extracting features from the class with small sample size; ContrastNet performs better than AAE and VAE in OA and AA when the number of samples is balanced. When the number of samples is imbalanced, ContrastNet tends to get higher OA and lower AA than AAE and VAE. 




\subsubsection{Visualization Experiments}

To intuitively show the clustering effect of ContrastNet, we use t-SNE \cite{TSNE} method to visualize the features extracted by AAE, VAE, and ContrastNet. The visualizations are shown in Fig. \ref{fig:tsne_IP}, \ref{fig:tsne_PU}, \ref{fig:tsne_SA}. In Fig. \ref{fig:tsne_IP}, it is a little hard to tell which feature distribution is better for classification in the IP dataset, and our experiments also proved that. \dd{Features in the PU dataset are shown in Fig. \ref{fig:tsne_PU}, clustering effect is obvious in the ContrastNet feature distribution, such as the features in class 0 and 8.} Features in the same class tend to be close to each other in the ContrastNet, which is due to the clustering algorithm in ContrastNet. Similarly, features in the SA dataset are shown in Fig. \ref{fig:tsne_SA}. \dd{AAE features in class 7 and VAE features in class 1 are mixed with other classes. However, they are both separated from other classes when they become contrast features.} This is a good illustration of our method's advantage. As a result, we can roughly make a conclusion that ContrastNet has the ability to decrease the inner-class distances and increasing the inter-class distances.

\begin{figure*}
\centering
\subfloat[AAE]{\includegraphics[width=2.2in]{IP_AAE_Features.png}
\label{fig:tsne_IP_AAE}}
\subfloat[VAE]{\includegraphics[width=2.2in]{IP_VAE_Features.png}
\label{fig:tsne_IP_VAE}}
\subfloat[ContrastNet]{\includegraphics[width=2.2in]{IP_ContrastFeature.png}%
\label{fig:tsne_IP_Contrast}}
\caption{Visualization of extracted features in the Indian Pines dataset. Each class is corresponding to a kind of color.}
\label{fig:tsne_IP}
\end{figure*}


\begin{figure*}
\centering
\subfloat[AAE]{\includegraphics[width=2.2in]{PU_AAE_Features.png}
\label{fig:tsne_PU_AAE}}
\subfloat[VAE]{\includegraphics[width=2.2in]{PU_VAE_Features.png}
\label{fig:tsne_PU_VAE}}
\subfloat[ContrastNet]{\includegraphics[width=2.2in]{PU_ContrastFeature.png}%
\label{fig:tsne_PU_Contrast}}
\caption{Visualization of extracted features in the University of Pavia dataset. Each class is corresponding to a kind of color.}
\label{fig:tsne_PU}
\end{figure*}

\begin{figure*}
\centering
\subfloat[AAE]{\includegraphics[width=2.2in]{SA_AAE_Features.png}
\label{fig:tsne_SA_AAE}}
\subfloat[VAE]{\includegraphics[width=2.2in]{SA_VAE_Features.png}
\label{fig:tsne_SA_VAE}}
\subfloat[ContrastNet]{\includegraphics[width=2.2in]{SA_ContrastFeature.png}%
\label{fig:tsne_SA_Contrast}}
\caption{Visualization of extracted features in the Salinas dataset. Each class is corresponding to a kind of color.}
\label{fig:tsne_SA}
\end{figure*}


\begin{figure*}
\centering
\includegraphics[width=4in]{oa_IP.pdf}

\caption{Parameter analysis based on the IP dataset. When altering the temperature value and window size, the performance of different modules are different. In this figure, $\tau$ means the temperature parameter in Eq. \ref{eq:infoNCE}, and horizontal axis is the window size for input patches.}
\label{fig:parameter}
\end{figure*}

\subsubsection{Parameter Analysis}

\dd{The window size and temperature value $\tau$ may affect the performance of our models, so we conducted some parameter analysis experiments. We vary the value of $\tau$ in $[0.01, 0.05, 0.1]$, and vary the window size in $[19, 21, 23, 25, 27]$. With different parameters, we recorded the OA of classification results in the IP dataset. Similar to the classification experiments before, we use 10\% labels and features for training the SVM and the rest for testing. As Fig. \ref{fig:parameter} shows, classification results of contrast features are significantly better than AAE features and VAE features with all kinds of parameters. The value of $\tau$ only affects the contrast features, so VAE features and AAE features do not show relevance with $\tau$. The performance of contrast features is relevant to $\tau$ when training the ContrastNet. It is not hard to tell from the figure that when $\tau=0.01$, contrast features can get the best classification results.
Moreover, when the window size increases, performances of VAE features and AAE features become better. It may owe to the increase of spatial information in patches. However, the change of window size does not make a tremendous difference in contrast features' performance. Because ContrastNet can get valuable information from contrastive learning, and the contribution of increased spatial information is relatively limited. These experiments show that ContrastNet is a robust and parameter-insensitive model. }

\subsubsection{Computational Aalysis}
The computational analysis is shown in Table \ref{tab:time}. Because the training of ContrastNet demands extracted AAE and VAE features, the training time of ContrastNet is considerably longer than other algorithms. However, when extracting features, the time consumption of ContrastNet is fairly fast than others. Because for AAE and VAE, only encoders are used in the feature extraction phase. Moreover, the structure of   AAE and VAE is relatively simple and efficient, so the ContrastNet performs fast in the feature extraction phase.

\begin{table*}
\caption{Computational analysis of different feature extration algorithms. The best value in each row is in bold. And the methods in bold are structures proposed in this paper. Some of the data in the table is quoted from \cite{3DCAE}.}
\label{tab:time}
\centering
\begin{tabular}{cccccccc}
\hline
\multicolumn{8}{c}{Indian Pines dataset}                                                                                     \\ \hline
\multicolumn{1}{c|}{}                       & 1D-CNN        & S-CNN & TPCA & SSAE          & EPLS   & 3DCAE & \textbf{ContrastNet}    \\ \hline
\multicolumn{1}{c|}{Training(s)}            & \textbf{20.6} & 119   & 44   & 240.1         & 111.9  & 1156  & 2073           \\ \hline
\multicolumn{1}{c|}{Inference (s)} & 17.4          & 3.2   & 150  & \textbf{2.76} & 47.3   & 5.22  & 12.77          \\ \hline
\multicolumn{8}{c}{Salinas dataset}                                                                                   \\ \hline
\multicolumn{1}{c|}{}                       & 1D-CNN        & S-CNN & TPCA & SSAE          & EPLS   & 3DCAE & \textbf{ContrastNet}    \\ \hline
\multicolumn{1}{c|}{Training(s)}            & \textbf{43.1} & 134   & 241  & 513           & 103.5  & 1159  & 4784           \\ \hline
\multicolumn{1}{c|}{Inference (s)} & 83.8          & 62    & 816  & \textbf{16.3} & 192.2  & 26.4  & 36.65          \\ \hline
\multicolumn{8}{c}{University of Pavia dataset}                                                                                 \\ \hline
\multicolumn{1}{c|}{}                       & 1D-CNN        & S-CNN & TPCA & SSAE          & EPLS   & 3DCAE & \textbf{ContrastNet}    \\ \hline
\multicolumn{1}{c|}{Training(s)}            & \textbf{32.1} & 332   & 44   & 491           & 127.13 & 1168  & 3778           \\ \hline
\multicolumn{1}{c|}{Inference (s)} & 150.07        & 106   & 150  & 31.9          & 141.5  & 32.04 & \textbf{27.82} \\ \hline
\end{tabular}
\end{table*}
\end{comment}

\section{Conclusion}
In this paper, we proposed an unsupervised feature learning method based on autoencoder and contrastive learning. This method combines unsupervised representative methods and unsupervised discriminative methods, learning to extract better features for hyperspectral classification than other baseline methods. In the proposed method, we designed two efficient autoencoder structure: VAE and AAE, and designed a model named ContrastNet for contrastive learning, which reduces the computing resources demand of contrastive learning. In fact, the VAE and AAE modules can be replaced by any other feature extraction algorithms. Our experiments show that the proposed method can extract more representative features and keep a high feature extraction speed in the testing phase. Our work shows that unsupervised learning still has great potential in the remote sensing field, and we hope others can get more exciting ideas through our exploration.
